Stealing Training Data from Large Language Models in Decentralized Training through Activation Inversion Attack

Decentralized training has become a resource-efficient framework to democratize the training of large language models (LLMs). However, the privacy risks associated with this framework, particularly due to the potential inclusion of sensitive data in training datasets, remain unexplored. This paper identifies a novel and realistic attack surface: the privacy leakage from training data in decentralized training, and proposes \textit{activation inversion attack} (AIA) for the first time. AIA first constructs a shadow dataset comprising text labels and corresponding activations using public datasets. Leveraging this dataset, an attack model can be trained to reconstruct the training data from activations in victim decentralized training. We conduct extensive experiments on various LLMs and publicly available datasets to demonstrate the susceptibility of decentralized training to AIA. These findings highlight the urgent need to enhance security measures in decentralized training to mitigate privacy risks in training LLMs.

==> tables/attack_model.tex <==
\begin{table}[ht]
\centering
\caption{The Impact of Attack Model Architecture on Attack Performance. Each attack model is configured with 6 decoder layers. The results are presented in terms of PPL.}
\label{tab:attack_model}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc|cccc}
\toprule[2pt]
\multirow{2}{*}{Victim Model} & \multirow{2}{*}{Attack Model Architecture} & Shadow Datasets & \multicolumn{4}{c}{Victim Datasets}      \\
                              &                                            & wikitext        & PIIs    & openwebtext & arxiv   & pile   \\ \hline
\multirow{3}{*}{GPT2-xl}      & Mistral                                    & 1.53            & 117.45  & 44.14       & 109.31  & 24.54  \\
                              & Qwen2.5                                    & 1.71            & 410.47  & 115.35      & 301.26  & 68.74  \\
                              & Gpt2                                       & 1.54            & 4.17    & 2.61        & 3.81    & 1.70   \\ \hline
\multirow{3}{*}{Bloom7b1}     & Mistral                                    & 1.54            & 7277.80 & 537.97      & 1203.97 & 445.71 \\
                              & Qwen2.5                                    & 1.48            & 7404.53 & 839.47      & 1947.76 & 651.55 \\
                              & Bloom                                      & 1.41            & 16.81   & 9.14        & 13.45   & 2.12   \\ \hline
\multirow{3}{*}{Llama3-8B}    & Mistral                                    & 2.60            & 2016.21 & 447.20      & 692.70  & 134.76 \\
                              & Qwen2.5                                    & 2.89            & 1810.44 & 549.28      & 1315.82 & 151.34 \\
                              & Llama                                      & 1.85            & 12.57   & 4.16        & 10.11   & 2.03   \\ \bottomrule[1.5pt]

\end{tabular}
}
\end{table}

==> tables/attack_model_backup.tex <==
\begin{table}[ht]
\centering
\caption{The Impact of Attack Model Architecture on Attack Performance. Each attack model is configured with 6 decoder layers. The results are presented in terms of PPL.}
\label{tab:attack_model}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc|cccc}
\toprule[2pt]
\multirow{2}{*}{Victim Model} & \multirow{2}{*}{Attack Model Architecture} & Shadow Datasets & \multicolumn{4}{c}{Victim Datasets}      \\
                              &                                            & wikitext        & PIIs    & openwebtext & arxiv   & pile   \\ \hline
\multirow{3}{*}{GPT2-xl}      & Mistral                                    & 1.532434718     & 117.45  & 44.14       & 109.31  & 24.54  \\
                              & Qwen2.5                                    & 1.706356711     & 410.47  & 115.35      & 301.26  & 68.74  \\
                              & Gpt2                                       & 1.543291913     & 4.17    & 2.61        & 3.81    & 1.70   \\ \hline
\multirow{3}{*}{Bloom7b1}     & Mistral                                    & 1.535357756     & 7277.80 & 537.97      & 1203.97 & 445.71 \\
                              & Qwen2.5                                    & 1.481726069     & 7404.53 & 839.47      & 1947.76 & 651.55 \\
                              & Bloom                                      & 1.406107218     & 16.81   & 9.14        & 13.45   & 2.12   \\ \hline
\multirow{3}{*}{Llama3-8B}    & Mistral                                    & 2.603444049     & 2016.21 & 447.20      & 692.70  & 134.76 \\
                              & Qwen2.5                                    & 2.891224462     & 1810.44 & 549.28      & 1315.82 & 151.34 \\
                              & Llama                                      & 1.847734218     & 12.57   & 4.16        & 10.11   & 2.03  \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table}

==> tables/base_result_backup.tex <==
% tables.tex

\begin{table*}[ht]
\centering
\caption{Text reconstruction performance of GPT-2-XL, Bloom-7B1, and LLaMA3-8B on four datasets. For all metrics except PPL, higher values indicate better performance.}
\label{tab:base_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc|ccc|ccc|c}
\toprule[2pt]
% \hline
\multirow{2}{*}{Victim Model} & \multirow{2}{*}{Dataset} & \multirow{2}{*}{PPL} & \multicolumn{3}{c|}{Rouge}      & \multicolumn{3}{c|}{Bleu}      & \multirow{2}{*}{Cos} \\ \cline{4-9}
                              &                          &                      & Rouge1   & Rouge2   & RougeL    & Bleu1    & Bleu2    & Bleu4    &                      \\ \hline
\multirow{4}{*}{Gpt2-xl}      & PIIs                     & 3.725906             & 0.841048 & 0.735223 & 0.8410215 & 0.774037 & 0.70875  & 0.592534 & 0.892224133          \\
                              & openwebtext              & 3.085841             & 0.950554 & 0.904678 & 0.9499552 & 0.880708 & 0.841762 & 0.771285 & 0.93960005           \\
                              & arxiv                    & 5.4323               & 0.922451 & 0.851664 & 0.9221703 & 0.810106 & 0.746846 & 0.635178 & 0.921457529          \\
                              & pile                     & 1.653329             & 0.975146 & 0.952666 & 0.9750504 & 0.949503 & 0.928737 & 0.889234 & 0.966821373          \\ \hline
\multirow{4}{*}{Bloom-7b1}    & PIIs                     & 14.81717             & 0.798137 & 0.674937 & 0.7978248 & 0.672434 & 0.600199 & 0.470294 & 0.886732221          \\
                              & openwebtext              & 4.641352             & 0.95404  & 0.915793 & 0.9537754 & 0.89159  & 0.857451 & 0.796006 & 0.946343243          \\
                              & arxiv                    & 15.44747             & 0.906145 & 0.826    & 0.9049029 & 0.771668 & 0.696915 & 0.56063  & 0.898831427          \\
                              & pile                     & 2.085233             & 0.973114 & 0.950243 & 0.9729964 & 0.951068 & 0.931851 & 0.895551 & 0.953125775          \\ \hline
\multirow{4}{*}{Llama3-8b}    & PIIs                     & 7.363312             & 0.795092 & 0.674507 & 0.7949278 & 0.7294   & 0.661444 & 0.543186 & 0.772945046          \\
                              & openwebtext              & 6.500885             & 0.925383 & 0.876017 & 0.9250533 & 0.881682 & 0.842453 & 0.772228 & 0.879064202          \\
                              & arxiv                    & 9.255523             & 0.8769   & 0.783265 & 0.8763907 & 0.796799 & 0.725079 & 0.597177 & 0.82953918           \\
                              & pile                     & 2.180419             & 0.96168  & 0.934619 & 0.9616122 & 0.942509 & 0.923151 & 0.88692  & 0.920280755          \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table*}

==> tables/model_size_backup.tex <==

\begin{table}[ht]
\centering
\caption{The relationship between attack performance and model size on GPT-2 and Bloom models.}
\label{tab:model_size}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule[2pt]
\multirow{2}{*}{Victim Model}                & \multirow{2}{*}{Model Size}                & \multirow{2}{*}{Dataset} & \multicolumn{4}{c}{metrics}                  \\
                                             &                                            &                          & PPL      & RougeL   & Bleu4    & Cos         \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{Bloom}} & \multicolumn{1}{c|}{\multirow{4}{*}{560m}} & PIIs                     & 15.22383 & 0.755987 & 0.457282 & 0.838139415 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 4.064717 & 0.938392 & 0.748586 & 0.923049808 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 14.60279 & 0.889816 & 0.51994  & 0.85961163  \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 2.456154 & 0.96645  & 0.877252 & 0.940752149 \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{4}{*}{1b7}}  & PIIs                     & 10.23899 & 0.797749 & 0.517596 & 0.889451742 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 3.312171 & 0.959928 & 0.808306 & 0.952394247 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 9.825108 & 0.924558 & 0.575449 & 0.909008205 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 2.005449 & 0.978407 & 0.921748 & 0.957987487 \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{4}{*}{7b1}}  & PIIs                     & 12.06283 & 0.807838 & 0.482967 & 0.892486393 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 4.407988 & 0.955469 & 0.811341 & 0.951343954 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 14.34313 & 0.909909 & 0.575406 & 0.902299047 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 1.917344 & 0.975715 & 0.909905 & 0.957693934 \\ \hline
\multicolumn{1}{c|}{\multirow{12}{*}{Gpt2}}  & \multicolumn{1}{c|}{\multirow{4}{*}{355m}} & PIIs                     & 5.701567 & 0.795913 & 0.524454 & 0.747232139 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 4.688037 & 0.908615 & 0.655283 & 0.88812542  \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 11.843   & 0.873263 & 0.536423 & 0.85599041  \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 2.750636 & 0.947597 & 0.792603 & 0.929776967 \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{4}{*}{774m}} & PIIs                     & 4.295362 & 0.811497 & 0.557581 & 0.824348211 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 3.421124 & 0.927434 & 0.705367 & 0.910575986 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 8.791323 & 0.895183 & 0.595468 & 0.881273806 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 2.302663 & 0.963662 & 0.839735 & 0.942203701 \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{4}{*}{1.5b}} & PIIs                     & 3.442145 & 0.84758  & 0.616235 & 0.899535477 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & openwebtext              & 3.620709 & 0.946216 & 0.758725 & 0.937531054 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & arxiv                    & 5.163485 & 0.92431  & 0.674316 & 0.922491789 \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                      & pile                     & 1.65191  & 0.974825 & 0.889096 & 0.963663757 \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table}

==> tables/pii_attack_result_backup.tex <==

\begin{table*}[ht]
\centering
\caption{The attack success rates of all models in precisely recovering the seven PII types: fax, birthday, SSN, address, job, bitcoin, and UUID.}
\label{tab:pii_attack_result}
\begin{tabular}{cccccccc}
\toprule[2pt]
\multicolumn{1}{l}{}           & fax      & birthday & SSN      & address  & job      & bitcoin  & UUID     \\ \hline
\multicolumn{1}{c|}{Gpt2-xl}   & 0.248996 & 1        & 0.761044 & 0.556225 & 0.965863 & 0.216867 & 0.174699 \\
\multicolumn{1}{c|}{Bloom-7b1} & 0.478992 & 0.985294 & 0.567227 & 0.565126 & 0.981092 & 0.035714 & 0.037815 \\
\multicolumn{1}{c|}{Llama3-8b} & 0.195745 & 0.951064 & 0.376596 & 0.410638 & 0.889362 & 0.034043 & 0.097872 \\ \bottomrule[1.5pt]
\end{tabular}
\end{table*}

==> tables/pii_compare.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of the ASR between our method and baselines in stealing phone and email data.}
\label{tab:pii_compare}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule[2pt]
\multirow{2}{*}{Victim Model} & \multirow{2}{*}{method} & \multicolumn{2}{c}{ASR} \\
                              &                         & phone      & email      \\ \hline
\multirow{3}{*}{Gpt2-xl}      & True prefix             & 0          & 0.04       \\
                              & SPT                     & 0          & 0.02       \\
                              & ours                    & 0.25       & 0.55       \\ \hline
\multirow{3}{*}{Bloom-7b1}    & True prefix             & 0.01       & 0.18       \\
                              & SPT                     & 0          & 0.10       \\
                              & ours                    & 0.42       & 0.62       \\ \hline
\multirow{3}{*}{Llama3-8b}    & True prefix             & 0          & 0          \\
                              & SPT                     & 0          & 0          \\
                              & ours                    & 0.16       & 0.42       \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table}

==> tables/pii_compare_backup.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of the ASR between our method and baselines in stealing phone and email data.}
\label{tab:pii_compare}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule[2pt]
\multirow{2}{*}{Victim Model} & \multirow{2}{*}{method} & \multicolumn{2}{c}{ASR} \\
                              &                         & phone      & email      \\ \hline
\multirow{3}{*}{Gpt2-xl}      & True prefix             & 0          & 0.040201   \\
                              & SPT                     & 0          & 0.0181818  \\
                              & ours                    & 0.248996   & 0.5481928  \\ \hline
\multirow{3}{*}{Bloom-7b1}    & True prefix             & 0.005025   & 0.1809045  \\
                              & SPT                     & 0          & 0.1        \\
                              & ours                    & 0.418067   & 0.6155462  \\ \hline
\multirow{3}{*}{Llama3-8b}    & True prefix             & 0          & 0          \\
                              & SPT                     & 0          & 0          \\
                              & ours                    & 0.157447   & 0.4191489  \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table}
